Bi-tuning of Pre-trained Representations

It is common within the deep learning community to first pre-train a deep neural network from a large-scale dataset and then fine-tune the pre-trained model to a specific downstream task. Recently, both supervised and unsupervised pre-training approaches to learning representations have achieved remarkable advances, which exploit the discriminative knowledge of labels and the intrinsic structure of data, respectively. It follows natural intuition that both discriminative knowledge and intrinsic structure of the downstream task can be useful for fine-tuning, however, existing fine-tuning methods mainly leverage the former and discard the latter. A question arises: How to fully explore the intrinsic structure of data for boosting fine-tuning? In this paper, we propose Bi-tuning, a general learning framework to fine-tuning both supervised and unsupervised pre-trained representations to downstream tasks. Bi-tuning generalizes the vanilla fine-tuning by integrating two heads upon the backbone of pre-trained representations: a classifier head with an improved contrastive cross-entropy loss to better leverage the label information in an instance-contrast way, and a projector head with a newly-designed categorical contrastive learning loss to fully exploit the intrinsic structure of data in a category-consistent way. Comprehensive experiments confirm that Bi-tuning achieves state-of-the-art results for fine-tuning tasks of both supervised and unsupervised pre-trained models by large margins (e.g. 10.7\% absolute rise in accuracy on CUB in low-data regime).

==> text/ack.tex <==
\subsection*{Acknowledgments}
You may include other additional sections here.

==> text/boa.tex <==
\section*{Author Contributions}

If you'd like to, you may include  a section for author contributions as is done in many journals. This is optional and at the discretion of the authors.


%This work focus on the retraining of unsupervised pretrained representations. There is no obvious risk of ethical and future societal aspects.
%The proposed method can be used for the training of deep learning models. Researchers can get some inspiration from this work. The algorithm can work quite robust and is without data bias.


==> text/expri.tex <==
\iffalse

\bibliography{../ref/JZhong.bib}

\fi

\section{Experiments}

\subsection{Experimental Settings}
% datasets
We study retraining under CORE from unsupervised visual representations performed in several visual recognition datasets, including:
\textbf{CUB-200-2011}~\cite{cub200-WelinderEtal2010} is a dataset for fine-grained visual recognition, including 200 birds species;
\textbf{Stanford Dogs}~\cite{dogs-KhoslaYaoJayadevaprakashFeiFei_FGVC2011} contains images of $120$ breeds of dogs;
\textbf{Stanford Cars}~\cite{cars-KrauseStarkDengFei-Fei_3DRR2013} contains images of $196$ classes of cars;
\textbf{Oxford-IIIT Pet} ~\cite{pets-parkhi2012cats} consists of $37$ classes of pets and
\textbf{FGVC Aircraft} ~\cite{aircraft-maji2013fine} is a fine-grained benchmark containing $100$ different aircraft variants. Baselines we compared to are standard fine-tuning and fine-tuning with auxiliary unsupervised loss (InfoNCE as Eq. \ref{infonce}) following a GPT~\cite{radford2018improving,radford2019language} style.
To reveal that our method is more effective in low-data regime, for each dataset, we create four configurations which sample $25\%, 50\%, 75\%$ and $100\%$ training data randomly for each category respectively.

% hyper-parameters details
We use Resnet-50~\cite{he2016deep} pretrained on ImageNet~\cite{deng2009imagenet} via MoCo~\cite{he2019momentum} as our backbone network on pytorch. We add a new fully connected layer on the second last layer (after global average pooling) of MoCo as a classifier, training from scratch with learning rate set to be 10 times those fine-tuned layers, following a \emph{de facto} configuration in fine-tuning. Our keys generating mechanism implemented following the MoCo ~\cite{he2019momentum} style, which maintains double queues respectively and keeps hidden keys($2048$-d in Eq. \eqref{CCE}) and standard contrastive keys($128$-d in Eq. \eqref{snce}), both normalized by their L2-norm ~\cite{wu2018unsupervised}, also a momentum-updated encoder with momentum coefficient $m=0.999$ as default MoCo setting. For all datasets, we set queue size as $8,16,24,32$ samples each category corresponding to four dataset-size configurations respectively. The temperature $\tau$ in Eq. \eqref{snce} and Eq. \eqref{CCE} is set as $0.07$ ~\cite{wu2018unsupervised}. We don't adjust trade-off coefficient $\lambda_1, \lambda_2$ carefully, and both just use $1$ by default without extra clarifications. The data augumentation setting only include randomly croping and resize to a $224\times224$-pixel image.
We use SGD as our optimizer. The SGD weight decay is $0.0001$ and the SGD momentum is $0.9$. We use a mini-batch size of $64$ and an initial learning rate of $0.01$. We train for $27000$ iterations with learning rate multiplied by $0.1$ every $6000$ iterations. 

\begin{table*}[tbp]
	%\vspace{-10pt}
	\addtolength{\tabcolsep}{2pt}
	\centering
	\vskip 0.1in
	% \resizebox{\textwidth}{!}{%
	
	\begin{tabular}{cccccc}
	% {p{2.1cm}<{\centering}|c|p{1.5cm}<{\centering }p{1.5cm}<{\centering} p{1.5cm}<{\centering} p{1.5cm}<{\centering}}
		\toprule
		\multirow{2}*{Dataset} & \multirow{2}*{Method} & \multicolumn{4}{c}{Sampling Rates} \\
		& & $25\%$ & $50\%$ & $75\%$ & $100\%$ \\
		\midrule
		\multirow{3}*{Dogs}    & MoCo                 & $54.95\pm$0.08          & $68.38\pm$0.12          & $72.51\pm$0.11          & $			       75.57\pm$0.12          \\
		                       & MoCo*                & $54.47\pm$0.05         & $67.66\pm$0.12          & $73.07\pm$0.14          & $ 75.58\pm$0.20         \\
				       & \textbf{MoCo+CORE}   & $\textbf{59.28}\pm$0.13 & $\textbf{69.52}\pm$0.11 & $\textbf{73.25}\pm$0.07 & $\textbf{76.65}\pm$0.34  \\
		\midrule
		\multirow{3}*{CUB}     & MoCo                 & $38.57\pm$0.13          & $58.97\pm$0.16          & $69.55\pm$0.18          & $			       74.35\pm$0.18         \\
		                       & MoCo*                & $36.43\pm$0.17          & $57.62\pm$0.14          & $67.82\pm$0.05          & $			       72.95\pm$0.29         \\
				       & \textbf{MoCo + CORE} & $\textbf{49.25}\pm$0.23 & $\textbf{66.88}\pm$0.13 & $\textbf{74.27}\pm$0.05 & $\textbf{77.12}\pm$0.23  \\
		\midrule
		\multirow{3}*{Cars}    & MoCo                 & $62.40\pm$0.26          & $81.55\pm$0.36          & $88.07\pm$0.19          & $			       89.81\pm$0.48         \\
				       & MoCo*                & $65.83\pm$0.27          & $82.39\pm$0.17          & $88.62\pm$0.11          & $			       90.56\pm$0.18         \\
				       & \textbf{MoCo + CORE} & $\textbf{69.44}\pm$0.32 & $\textbf{84.41}\pm$0.07 & $\textbf{89.32}\pm$0.23 & $\textbf{90.88}\pm$0.13  \\
		
		\midrule
		\multirow{3}*{Pet}     & MoCo                 & $70.88\pm$0.44          & $80.68\pm$0.12          & $84.40\pm$0.18          & $			       86.30\pm$0.30         \\
				       & MoCo*                & $71.08\pm$0.29          & $79.81\pm$0.05          & $83.49\pm$0.12          & $			       85.69\pm$0.05       \\
				       & \textbf{MoCo + CORE} & $\textbf{74.13}\pm$0.66 & $\textbf{82.94}\pm$0.32 & $\textbf{86.09}\pm$0.33 & $\textbf{87.79}\pm$0.49  \\
		\midrule
		\multirow{3}*{Aircraft}& MoCo                 & $58.98\pm$0.54          & $77.39\pm$0.31          & $84.82\pm$0.24          & $			       87.35\pm$0.17         \\
				       & MoCo*                & $60.70\pm$0.08          & $78.93\pm$0.17          & $85.09\pm$0.10          & $			       87.56\pm$0.15         \\
				       & \textbf{MoCo + CORE} & $\textbf{63.16}\pm$0.26 & $\textbf{79.98}\pm$0.22 & $\textbf{86.23}\pm$0.29 & $\textbf{88.55}\pm$0.38 \\
		\bottomrule

	\end{tabular}

	\caption{Comparison of Top-1 Accuracy on Different Datasets using ResNet-50 as the backbone and pretrained by MoCo. Averaged over 5 trials. Here (i) MoCo is retraining straightforward; (ii) MoCo* is retraining with InfoNCE; (iii) MoCo + CORE is retraining under CORE framework.}
	\label{table:result}

\end{table*}

\subsection{Result and Analysis}
\label{resandana}

\paragraph{Results.} Table~\ref{table:result} shows the top-1 classification accuracies on $5$ differents recognition datasets. CORE consistently improves performances of retraining from unsupervised representations (pretrained by MoCov1~\cite{he2019momentum} here). Even in $100\%$ sample ratio configurations, CORE can bring significant gains. Note that borrowing fine-tuning strategy in GTP~\cite{radford2018improving} trivially brings limited benefits even harmful in some datasets (e.g. CUB) with a small optimal coefficient of $\lambda$ ($0.01$ while $1$ in CORE).
\vspace{-10pt}
\paragraph{Ablation: Collaborative Effects.} Table~\ref{table:colla} shows the results finetuned on \textbf{CUB}~\cite{cub200-WelinderEtal2010}, choosing some different loss combinations among CE, CCL and MCE. Only using either CCL or MCE with CE makes little influence. These experiments proved that there is some collaborative effect of CCL and MCE empirically. It is worth to mentioning that CCL and MCE can work independently of CE, while we optimize these three losses simultaneously get the best result. As discussed in previous sections, we speculate that CORE helps retrained model characterize the joint distribution of training data when using both CCL and MCE.

\begin{table*}[tbp]
	\addtolength{\tabcolsep}{2pt}
	\centering
	\begin{tabular}{ccccccc}
	  \toprule
	  \multicolumn{3}{c}{Three Losses}  & \multicolumn{4}{c}{Sample Rate} \\
	  CE & CCL & MCE & $25\%$ & $50\%$ & $75\%$ & $100\%$\\
	  \midrule
	  \ding{51} & \ding{55}& \ding{55}  & $38.57\pm$0.13          & $58.97\pm$0.16          & $69.55\pm$0.18          & $			       74.35\pm$0.18         \\
	  \ding{51} & \ding{51}& \ding{55} &$41.09\pm$0.23 &$60.77\pm$0.31 &$70.30\pm$0.29 & $74.30\pm$0.2 \\
	  \ding{51} & \ding{55}& \ding{51} &$39.51\pm$0.11 &$59.20\pm$0.18 &$69.26\pm$0.12 & $74.80\pm$0.12 \\
	  \ding{55} & \ding{51}& \ding{51} &$47.70\pm$0.41 &$64.77\pm$0.15 &$71.69\pm$0.11 & $76.54\pm$0.24 \\
	  \ding{51} & \ding{51}& \ding{51} & $\textbf{49.25}\pm$0.23 & $\textbf{66.88}\pm$0.13 & $\textbf{74.27}\pm$0.05 & $\textbf{77.12}\pm$0.23  \\
	  \bottomrule
	  
 	\end{tabular}
 
	\caption{Collaborative effect in CORE on CUB-200-2011 using ResNet-50 as the backbone and pretrained by MoCo. We compare the results with different sample rate.}
	\label{table:colla}
\end{table*}

\paragraph{Ablation: Keys Numbers.} 
% #key
Previous works ~\cite{he2019momentum,chen_simple_2020} reveal that a large amount of negatives benefit to contrastive learning. In CORE, we report results under different choices of the number of keys. Table \ref{table:ksm} shows the sensitivity of numbers of sampling keys in CORE (MoCo) under 4 sampling ratio configurations. Note that CUB has a various categories with a few images in each category, we let K balanced sampled from every category to simplify our analysis here.  
Table \ref{table:ksm} shows that though a larger key pool is beneficial, we can not expand the key pool limited to insufficient training data, which may lose sampling stochasticity during training. This result suggests that there is a trade-off between stochasticity and a large of number keys. 
% Mechanism


\begin{table*}[!htbp]
	\centering
	\addtolength{\tabcolsep}{2pt}
	\centering
	
	%\vspace{-3pt}
	\begin{tabular}{cccccccc}
	  \toprule
	  K per class   &1                & 2               &    4           &  8            & 16         &  32     & 64          \\
	  \midrule
	  25\%          & $48.93$	  & $49.25$         & $49.09$        & $47.94 $      & $47.65$    & $47.78$ & $44.10$     \\
	  100\%         & $75.90$         & $76.45$         & $76.26$        & $76.41$       & $76.40$    & $77.12$ & $76.23$     \\

	  % retraining    & $90.55\pm$0.20  & $90.65\pm$0.15  & $90.77\pm$0.23 & $90.79\pm$0.23& $90.81\pm$0.06       & $91.01\pm$0.26\\
	  
	  \bottomrule
 	\end{tabular}
 	%}
	\caption{Comparison of different numbers of sampled keys, on 25\% and 100\% ratio of CUB (200 categories), indicates that there exists a trade-off between sampling stochasticity and a large number keys. (backbone ResNet50 via MoCo). Note that keys may be duplicate when the number of sampled keys is larger than dataset size. Standard deviations are omitted here to save space, please refer to the full table in the  \textit{Appendix}.}
	\label{table:ksm}
	% \vspace{-10pt}
\end{table*}

\paragraph{Ablation: different representations} CORE is a framework for unsupervised representations. we evaluate CORE on MoCov1, MoCov2 (ResNet50)~\cite{he2019momentum}, SimCLR~\cite{chen_simple_2020} (ResNet50 1x, 2x models, corresponding to the "$\times 8$", "$\times 16$" cases in ~\cite{kolesnikov2019revisiting} because the standard-sized ResNet is referred to as "$\times 4$" in ~\cite{kolesnikov2019revisiting}), InsDisc ~\cite{wu2018unsupervised} on Cars (100\% sampling ratio). As shown in Table \ref{table:different} CORE consistently improves the baselines.

\begin{table*}[!htbp]
	\addtolength{\tabcolsep}{2pt}
	\centering
	
	%\vspace{-3pt}
	\begin{tabular}{ccccccc}
	  \toprule
	  Methods     & MoCov1     & MoCov2 &  SimCLR(1x) & SimCLR(2x) & InsDisc \\
	  \midrule
	  Retraining  & $89.81\pm$0.48            & $90.15\pm$0.17        &   $89.30\pm$0.18     &   $91.22\pm$0.14          &     $86.59\pm$0.22     \\
	  CORE        & $\textbf{90.88}\pm$0.13   & $\textbf{90.79}\pm$0.13 &   $\textbf{90.84}\pm$0.22     &   $\textbf{91.93}\pm$0.19        &  $\textbf{89.54}\pm$0.25   \\
	  \bottomrule
 	\end{tabular}
	\caption{Top-1 accuracies on Cars with different representations (\%)}
	\label{table:different}
	% \vspace{-10pt}
\end{table*}

\begin{table*}[!htbp]
	\addtolength{\tabcolsep}{2pt}
	\centering
	
	%\vspace{-3pt}
	\begin{tabular}{ccccccc}
	  \toprule
	  dim           &32               & 64              &    128         &  256          & 512                  & 1024          \\
	  \midrule
	  from scratch  & $90.55$ 	  & $90.65$         &  $90.78$       & $90.79$       & $90.81$              & $91.01$       \\
	  retraining    & -               & -               &  $90.88$       & -             &  -                   & -              \\

	  % retraining    & $90.55\pm$0.20  & $90.65\pm$0.15  & $90.77\pm$0.23 & $90.79\pm$0.23& $90.81\pm$0.06       & $91.01\pm$0.26\\
	  \bottomrule
 	\end{tabular}
% 	\vspace{+2pt}
	\caption{Top-1 accuracies on Cars with different projection head $g(\cdot)$ (backbone ResNet50 pretrained via MoCo) (\%). Here ‘-’ denotes that these results are not available since the dimension of MoCo is $128$. Note that standard deviations are omitted here to save space, full table see supplements.}
	\label{table:dim}
	% \vspace{-10pt}
\end{table*}

\paragraph{Ablation: the Projector in CORE} Table \ref{table:dim} shows ablation study result of projection head $g(\cdot)$. it is not sensitive to projection head $g(\cdot)$ under this experiment setting. Though limited, it show a similar trend of projection dim to~\cite{chen_simple_2020} that a larger dim of projection head $g(\cdot)$ is optional.
Note that some unsupervised pretraining methods with contrastive loss have a projector in nature. So that CORE can borrow these parameters instantly. If pretrained models don't provide these parameters. Table \ref{table:dim} shows that it doesn't matter whether initialize the project layer or not.

\paragraph{Visualization.}  T-SNE~\cite{maaten2008visualizing} visualization of different baseline retrained on Pets~\cite{pets-parkhi2012cats} 100\%. Visualization of the validation set shows as Fig. \ref{fig:TSNE}. Note that representations in \ref{fig:tsne-moco} do not present good classification structures. $\ref{fig:tsne-ce-bsl}$ suggests that forcely introduce $p(x)$ modeling may cause conflict with $p(y|x)$ modeled by CE. $\ref{fig:tsne-core}$ suggests CORE model $p(x)$ and $p(y|x)$ with consistency.
Though limited accuaracy, some cluster shows in Fig. \ref{fig:TSNE} may not clear. CORE presents better structures.

\begin{figure}[!htbp]
\centering
\subfigure[MoCo]{
		\includegraphics[width=0.23\textwidth]{src/pet_bsl_3.pdf}
		\label{fig:tsne-moco}
}
\subfigure[CE]{
		\includegraphics[width=0.23\textwidth]{src/pet_ce_3.pdf}
		\label{fig:tsne-ce}
}
\subfigure[CE + InfoNCE]{
		\includegraphics[width=0.23\textwidth]{src/pet_ce+bsl_3.pdf}
		\label{fig:tsne-ce-bsl}
}
\subfigure[CORE]{
		\includegraphics[width=0.23\textwidth]{src/pet_combine_3.pdf}
		\label{fig:tsne-core}
}
\caption{ T-SNE \cite{maaten2008visualizing} visualization of different baseline on Pets~\cite{pets-parkhi2012cats}.}
\label{fig:TSNE}
\end{figure}%
\vspace{-10pt}

\section{Conclusion}
%Remarkable advances have been witnessed in unsupervised pretrained models, but it remains unclear how to leverage the knowledge of unsupervised models to downstream classification tasks. 
In this paper, we propose a novel {Co}ntrastive {Re}training (CORE) to fulfill this \textit{blank area }of deep learning community. CORE jointly model marginal and conditional distribution in a unified framework. Further, we propose a category-aware contrastive learning loss to tailor the commonly used unsupervised contrastive loss into a supervised retraining paradigm and a manifold-aware supervised learning loss to consider the manifold structure in the supervised retraining classifier. Extensive experiments and ablation studies demonstrate the effectiveness of CORE and the effectiveness of our proposed novel loss functions.

